Identification of structures driving trailing-edge noise. Part II -- Numerical investigation

The aim of the present work is to investigate the mechanisms of broadband trailing-edge noise generation to improve prediction tools and control strategies. We focus on a NACA 0012 airfoil at 3 degrees angle of attack and chord Reynolds number Re = 200,000. A high-fidelity wall-resolved compressible implicit large eddy simulation (LES) is performed to collect data for our analysis. The simulation is designed in close alignment with the experiment described in detail in the companion paper (Demange et al. 2024b). Zig-zag geometrical tripping elements, added to generate a turbulent boundary layer, are meshed to closely follow the experimental setup. A large spanwise domain is used in the simulation to include propagative acoustic waves with low wavenumbers. An in-depth comparison with experiments is conducted showing good agreement in terms of mean flow statistics, acoustic and hydrodynamic spectra, and coherence lengths. Furthermore, a strong correlation is found between the radiated acoustics and spanwise-coherent structures. To investigate the correlation for higher wavenumbers, spectral proper orthogonal decomposition (SPOD) is applied to the spanwise Fourier-transformed LES dataset. The analysis of all SPOD modes for the leading spanwise wavenumbers reveals streamwise-travelling wavepackets as the source of the radiated acoustics. This finding, confirming observations from experiments in the companion paper, leads to a new understanding of the turbulent structures driving the trailing-edge noise. By performing extended SPOD based on the acoustic region, we confirm the low rank nature of the acoustics, and a reduced-order model based on acoustic extended SPOD is proposed for the far-field acoustic reconstruction.

==> colors_authors.tex <==
% \usepackage[dvipsnames,table,xcdraw]{xcolor}

% Use the color defined here to differentiate between authors
% For each authors write, underline, bar
% OliveGreen, blue, violet, OrangeRed, Mulberry

% S. Demange
\newcommand{\SD}[1]{{\color{OliveGreen} #1}} 
\newcommand{\SDt}[1]{{\color{OliveGreen} \st{#1}}}
\newcommand{\SDu}[2][OliveGreen]{\setulcolor{#1}\ul{#2}\setulcolor{OliveGreen}}

% S. Jekosch
\newcommand{\SJ}[1]{{\color{blue} #1}} 
\newcommand{\SJt}[1]{{\color{blue} \st{#1}}}
\newcommand{\SJu}[2][blue]{\setulcolor{#1}\ul{#2}\setulcolor{blue}}

% B Church
\newcommand{\BC}[1]{{\color{violet} #1}} 
\newcommand{\BCt}[1]{{\color{violet} \st{#1}}}
\newcommand{\BCu}[2][violet]{\setulcolor{#1}\ul{#2}\setulcolor{violet}}
